Non-Binary Gender Expression in Online Interactions

Many openly non-binary gender individuals participate in social networks. However, the relationship between gender and online interactions is not well understood, which may result in disparate treatment by large language models. We investigate individual identity on Twitter, focusing on gender expression as represented by users chosen pronouns. We find that non-binary groups tend to receive less attention in the form of likes and followers. We also find that nonbinary users send and receive tweets with above-average toxicity. The study highlights the importance of considering gender as a spectrum, rather than a binary, in understanding online interactions and expression.

==> intro.tex <==

%Identity is fundamental to how individuals define themselves internally, and how they present themselves to others~\cite{deaux1993reconstructing}. 
%`Identity' is defined along multiple dimensions including age, gender, race, ethnic origin, socio-economic status, sexual orientation and political ideology.
An individual's identity, defined along multiple dimensions such as age, gender, race, ethnic origin, socio-economic status, etc., influences how they express themselves, and how they experience others within their social interactions ~\cite{deaux1993reconstructing}. 
As social interactions continue to migrate online, social media platforms play an increasingly critical role in identity formation~\cite{polletta2001collective,manago2015identity}. One aspect of online identity that has received significant attention from social media researchers is collective identity, which manifests itself through people joining social movements. Collective identity can become visible online when people adopt certain hashtags, such as \#metoo or \#blacklivesmatter in social media posts or in their online profiles. 
Using hashtags as markers of online collective identity, researchers have studied how these identities organize themselves within social hierarchies~\cite{barron2022quantifying}, who they interact with, and what they talk about~\cite{chang2022justiceforgeorgefloyd,khazraee2018digitally}. However, while individual identity overlaps with collective identity, it is not synonymous with it and requires further study.

% Importance of understanding language cues
Recent advances in natural language processing (NLP) provide new tools for the study of identity in online platforms~\cite{pathak2021method}. Language conveys not just the meaning of online conversations but also its emotional tone and moral sentiment~\cite{emotion_moral}. Emotions expressed in text messages can affect the others' feelings even without visual cues (e.g., facial expressions) or audio signals (e.g., tone of voice)~\cite{kramer2014experimental}. Language cues capture hostility, threats, personal attacks, and other dimensions of toxic speech~\cite{chen2012detecting,waseem-etal-2017-understanding}. 

% Gender is non-binary and underlooked
We study individual identity on the Twitter platform and how it mediates online expression and interactions, with a specific focus on gender.
%We focus on gender, one of the core dimensions of individual identity. 
Traditionally conceptualized in Western society as binary---specifically `male' vs `female'---two recent developments have transformed how we think about gender. First, there is growing recognition of gender as a cultural construct, distinct from the biologically-based sex; second, there is growing awareness that  gender forms a spectrum, rather than a binary identity. As a proxy of gender expression, we study pronouns users choose to display in their online profile or biography. %\footnote{
% \note{JA: The next two sentences are somewhat awkward} We understand that pronouns used are not directly indicative of gender labels. For that reason we are careful to group users by pronoun groups, which is a form of gender identity while different from labels.
%$} 
These pronouns range from the traditional binary gender categories (`she/her' %representing a `woman' 
and `he/him')
%representing a `man', 
to non-binary and gender nonconforming~\cite{hicks-etal-2016-analysis} categories (they/them', `she/ze', `she/they/xe', etc.). We study eight pronoun groups with the most members, revealing the spectrum of gender identity online (See \S \ref{data} for more details). 

% The need to include non-binary users in the toxicity/emotion metrics!
%The following hypothesis drives our research questions: \textit{online communities are less welcoming to gender minorities, whose contributions are ignored or minimized, and who receive replies that are more toxic and express  more negative emotions.} 
It is crucial to create positive online spaces for sexual and gender minority people. 
Gender-queer populations are at a higher risk of workplace discrimination, social isolation and shortened lifespan~\cite{tabaac2018discrimination}.
Additionally, LGTBQ+ youth are more likely to participate in online LGBTQ+ communities than real life communities~\cite{mcinroy2019lgbtq}.
% , making it crucial to create positive online spaces for them. %information exploration and social support. 
To explore how welcoming online communities are to non-binary populations, we investigate the following research questions:
%Misogynistic hate speech has a chilling effect on women and people of color, discouraging them from speaking up~\cite{carlson2017misogynistic}. 
%
%In this work, we will "use ‘trans’ broadly to refer to transgender, transsexual, gender nonconforming, gender variant, and non-binary individuals” \cite{hicks-etal-2016-analysis}. 

%We look at how individual processes on Twitter (activity, attention, emotion and toxicity in tweets/replies) vary with social identity (pronouns, gender). 

\begin{description}
%    \item What are the differences in user activity (Twitter post counts, like counts and following counts) by user pronoun groups?
%    \item What are the differences in user attention (percent of users verified, number of followers, number verified) and tweet attention (number of retweets, favorites and replies) by user pronoun groups?
    \item[RQ1] How do users in different pronouns groups vary in their level of online activity and the online attention they %and their posts 
    receive from others?  
%    \item[RQ2] Which user pronoun groups convey more positive and/or negative emotions on Twitter?
    \item[RQ2] What are the differences in the emotions expressed by different user pronoun groups? Which groups
    %Do the minority pronouns groups 
    receive more negative replies? 
    \item[RQ3] Which user pronoun groups convey more toxicity on Twitter? Which groups experience more toxicity from others?
%    \item[RQ4] What effect does user gender, tweet emotion and tweet toxicity have on the emotion and toxicity in the replies to the tweet?
\end{description}

%We operationalize the research questions through the following proxies. 
As a measure of online \textit{activity} we use number of messages a user posts and likes, and number of people followed.
%posted, liked by others, and the following count. 
Similarly, we measure the \textit{attention} group members receive as %share of verified accounts, 
the average number of retweets and likes of own messages
%, share of own messages with replies, 
 and followers count.
%We use state-of-the-art emotion and toxicity detection methods to quantify the presence of positive and negative emotions and toxicity in a group members' tweets and replies they receive from others.
We use state-of-the-art NLP models to automatically quantify a range of emotions expressed in text, such as joy, anger, fear and disgust~\cite{alhuzali2021spanemo}. In addition to affect, we use NLP models to detect toxicity in language~\cite{Detoxify}, enabling us to study social inclusion and exclusion at scale.


%\note{Summary of what we found}
%In line with our hypothesis,
We find that %gender-queer groups tend to be more vocal than binary groups, preferring to post messages rather than liking them. Additionally, 
while non-binary groups 
% receive more replies, 
are equally active online, their messages get less attention through likes. We also find interesting variation in emotions expressed by different groups, and the emotionality of replies to their messages. In particular, gender-queer groups tend to express more positive emotions in their tweets and fewer negative emotions. This is %though there are a few notable exceptions. This 
in contrast to binary groups who express more positive emotions and fewer negative emotions. 
%In line with our hypothesis, 
Non-binary users tend to receive fewer positive replies to their tweets. 
We find that non-binary groups also post more toxic messages. 
We hope that by treating gender expression as a spectrum and not a binary category we improve accuracy of computational methods which analyze gender equity and equality. 
%We suspect that this is due to non-binary users posting with more profanities than binary users.
%However, we do not yet have enough evidence to conclude whether that's an indicator of actual harmful interactions or the biases in toxicity detection algorithm.

%\note{JA: Kristina said take a stab, so....I'm not positive about any of this, I won't be offended if we don't use it.}
% Our work makes the following key contributions: First, we establish a data set of social media posts from users with fine-grained gender pronouns on their profile.
% By analyzing a wider spectrum of identity, we can more fully investigate the social media behavior and interactions of marginalized groups.
% Second, we provide an analysis of the activity, attention, toxicity and emotional content of each pronoun group, gaining a greater understanding of how members of each group interact, and are interacted with.
% Lastly, these results surface important questions about the nature of the NLP tools themselves, and how these tools may represent --- or potentially misrepresent --- different gender identities. 

%\note{Concluding sentences should focus on impact of the work. Perhaps moving towards fostering a more inclusive online environment, creating a more diverse workforce, etc}
%Our work makes the following contributions. First, we treat gender expression as a spectrum and not a binary category, allowing us to compare outcomes of computational tools across groups. 
%Additionally, by treating gender expression as a spectrum and not a binary category we improve accuracy of computational methods which analyze gender equity and equality. 
%Additionally, we explore the visibility and interactions in social media networks of people with historically marginalized gender identities. Finally, our work poses new research questions surrounding emotion and toxicity detection's ability to treat gender non-conforming users fairly. This will help improve the visibility of non-binary users in online communities and foster an environment that is welcoming to all forms of gender expression. %\note{JA: Given the effort spent distancing the association of pronouns with "Actual" gender, do we want to tie the whole thing to actual gender here at the end?} 



%Diverse workforce that includes all gender identities is more innovative and productive~\cite{Campbell2013, joshi2014whom}. 
%It is also better able to anticipate potential downstream harms of their products, such as unfair treatment by algorithms.


